Activity Driven Weakly Supervised Object Detection

Weakly supervised object detection aims at reducing the amount of supervision required to train detection models. Such models are traditionally learned from images/videos labelled only with the object class and not the object bounding box. In our work, we try to leverage not only the object class labels but also the action labels associated with the data. We show that the action depicted in the image/video can provide strong cues about the location of the associated object. We learn a spatial prior for the object dependent on the action (e.g. "ball" is closer to "leg of the person" in "kicking ball"), and incorporate this prior to simultaneously train a joint object detection and action classification model. We conducted experiments on both video datasets and image datasets to evaluate the performance of our weakly supervised object detection model. Our approach outperformed the current state-of-the-art (SOTA) method by more than 6% in mAP on the Charades video dataset.

==> tex/experiments.tex <==
\vspace{-0.3\baselineskip}
\section{Experiments}
\vspace{-0.3\baselineskip}
\label{sec:evaluation}

Our method is applicable to both the video and image domains. 
% The action driven weakly supervised detection task takes video clips or images with action labels as training samples, and is evaluated on test images, where object bounding boxes are annotated. 
We require datasets with human action labels for training and object bounding box annotations for evaluation.

%(1) the Charades dataset \cite{sigurdsson2016hollywood}, which consists of daily-life videos captured by hand-held devices and (2) HICO-DET dataset \cite{chao2018learning}, which contains images of various human-object interactions.

 \textbf{Video datasets}: The Charades dataset \cite{sigurdsson2016hollywood} includes 9,848 videos of 157 action classes, among which, 66 are interactive actions with objects. There are on average 6.8 action labels for one video. The official Charades dataset doesn't provide object bounding box annotations and we use the annotations released by \cite{yuan2017temporal}. 
In the released annotations, 1,812 test videos are down-sampled to 1 frame per second (fps) and 17 object classes are labeled with bounding boxes on these frames. There are 3.4 bounding box annotations per frame on average. We follow the same practice as in \cite{yuan2017temporal}: training on the 7,986 videos (54,000 clips) in training set and evaluate on 5,000 randomly selected test frames from 200 test videos.

The EPIC-KITCHENS \cite{Damen2018EPICKITCHENS} is a newly released ego-centric video dataset which is captured by head-mounted camera in different kitchen scenes. In the training data, the action class is annotated for 28,473 trimmed video clips and the object bounding boxes are labeled for 331 object classes. As the object bounding box annotations are not provided for the test splits, we divide the training data into training, validation and test parts. The top 15 frequent object classes (which are present in 85 action classes) are selected for experiments, resulting in 8,520 training, 1,000 validation and 200 test video clips. We randomly sample three times from each training clip and generate 28,560 training samples. We also randomly sample 1,200 test frames from the test clips. There are 1.46 object bounding box annotations per test frame on average.

\textbf{Image dataset} The HICO-DET dataset \cite{chao2018learning} is designed for human-object interaction (HOI) detection task. This dataset includes 38,118 training images and 9,658 test images. The human bounding box, object bounding box and an HOI class label are annotated for both training and test images. In total, there are 80 object classes (\eg~\textit{cup}, \textit{dog}, \etc) and 600 HOI classes (\eg~\textit{hold cup}, \textit{feed dog}, \etc).  We filter out all samples with ``no\_interaction'' HOI labels, interaction class with less than 20 training samples and all ``person'' as object class samples. This results in 32,100 training samples of 510 interaction classes and 79 object classes. We use the HOI labels as action class labels during training and the object bounding box annotations are used only for evaluation. Unlike Charades where the interactions mostly happen between one subject and one object, there are cases where multiple people interact with one object (\eg~``boarding the airplane'') and one person interacts with multiple objects (\eg~``herding cows''), which makes it more challenging to learn the object appearance.

We report per-class \textit{average precision} (AP) at \textit{intersection-over-union} (IoU) of 0.5 between detection and ground truth boxes, and also mean AP (mAP) as a combined metric, following the tradition of \cite{yuan2017temporal}. We also report \textit{CorLoc} \cite{deselaers2012weakly}, a commonly-used weakly supervised detection metric. CorLoc represents the percentage of images where at least one instance of the target object class is correctly detected (IoU\textgreater0.5) over all images that contain at least one instance of the class.

% The evaluation toolbox released by \cite{girshick2015fast} is slightly modified to adapt to Charades dataset. 
%The evaluation code in TensorFlow detection metric toolkit is directly used.
\vspace{-0.4\baselineskip}
\subsection{Implementation details}
\vspace{-0.4\baselineskip}
We use VGG-16 and ResNet-101 pre-trained on ImageNet dataset as our backbone feature extraction networks. All \textit{conv} layers in the network are followed with \textit{ReLU} activation except for the top classification layer. Batch normalization \cite{ioffe2015batch} is applied after all convolutional layers. In order to compute the classification scores ($s_O, s_A^H, s_A^O$), three branches are built on top of the last convolutional block. Each branch consists of ROI-pooling layer and 2-layer multiple layer perception (MLP) of intermediate dimension of 4096. The threshold for removing person proposal regions is set as $\theta_h=0.5$.
% For each action $a$, we estimate a weight vector of dimension $||P||$ as keypoint weight ($w_{key}^a$). A weighted sum of all keypoint locations is used as anchor location. The object location distribution parameters $\mu_a,\sigma_a$ (\equref{eqn:obj_weight}) are also estimated for each action to generate the location probability $w_r^a$.

% We model the spatial prior with estimating the keypoint weight $w_{key}^a$ (\equref{eqn:anchor}) and the object location probability distribution parameters $\mu_a,\sigma_a$ (\equref{eqn:obj_weight}). 

The Adam optimizer \cite{kingma2014adam} is applied with learning rate of $2\times 10^{-5}$ and batch size of $4$. The loss weights are set as $\alpha_a=1.0$, $\alpha_o=2.0$.
The number of sampled frames in a clip is set as $n=8$ and the number of proposals is set as $n_r=700$. The whole framework is implemented with PyTorch framework \cite{paszke2017automatic}. We train on a single Nvidia Tesla M40 GPU. The whole training converges around 20 hrs. More details of implementation are presented in supplemental material.


%To better understand the effectiveness of each module in our approach, we conducted comprehensive ablation experiments. On both Charades and HICO-DET datasets, different weakly supervised and semi-supervised training setups are evaluated. We also compared current SOTA methods and other baseline methods we proposed on these two datasets. As there is limited number of works which report object detection performance on these two datasets, we constructed our own baseline methods by incorporating person detection and pose estimation into other SOTA methods \cite{gkioxari2015finding,bilen2016weakly}. We acknowledge that there are stronger weakly supervised methods like \cite{} which incorporate more sophisticated approaches. However, here we only compare with these two baseline methods due to their simplicity and code availability. That being said, any of the more recent works can be easily extended with our idea for action driven object detection.
\vspace{-0.3\baselineskip}
\subsection{Ablation experiments}
\vspace{-0.4\baselineskip}
To explore how much each module contributes to the final performance, we investigate different variants of our framework: different distributions for modeling spatial location of object \wrt to the detected person and different loss term combinations. The different distributions include normal distribution and a fixed grid of probability values, where we make a discrete version of spatial prior module by pre-defining a $3\times 3$ grid around the keypoint, to replace the normal distribution. More details of this variant are presented in supplementary material.
% , and the size of each cell of the grid is fixed to be $64\times 64$. There is an estimated weight for each cell as attention and all proposals whose centers fall into the cell will be assigned with the attention weight. 

We also totally removed person detection bounding box and pose estimation from our pipeline to explore how much the object spatial prior helps in object localization (``Center'' as the prior method). For this baseline, we use the frame center as the anchor location $\src{L}$ and learn the $\mu_a$ and $\sigma_a$.
We experimented with different learning strategies for distribution based prior: learning distribution mean only ($\mu_a$), learning variance only ($\sigma_a$) and joint learning of mean and variance ($\mu_a+\sigma$). The supervision of the proposed pipeline comes in two aspects: object classification and action classification. We experimented with applying either one supervision signal or applying both loss terms. 

\begin{table}[]
\vspace{-0.8\baselineskip}
\fontsize{8}{9}\selectfont
% \def\arraystretch{1.5}
\setlength{\tabcolsep}{3pt}
\centering
\caption{Object detection performances of different variants on Charades}
\label{tbl:ab_study}
\begin{tabular}{l|c|c|c}
\specialrule{.2em}{.1em}{.1em}
 Spatial prior  & Loss term  & mAP  & CorLoc   \\ \hline
 Center            & action+object  & 3.43 & 34.27\\
 Grid              & action+object  & 4.32 &  36.94\\ \hline
 Distribution              & action  & 2.61 &  31.60\\
 Distribution              & object  & 5.86 &  39.24 \\
 Distribution              & action+object  &  \textbf{8.76}  & \textbf{47.91}\\ \hline

 Distribution ($\mu$)     & action+object  & 6.27  & 42.36\\ 
 Distribution ($\sigma$)     & action+object  & 4.86 & 38.05\\
 Distribution ($\mu + \sigma$)    & action+object  & \textbf{8.76} & \textbf{47.91}\\ \hline

% VGG-16    & Distribution      & action+object  & 6.87 \\
% ResNet-101 & Grid             & action+object  & 5.59 \\
% ResNet-101 & Distribution     & action+object  & \textbf{7.11} \\\hline
% VGG-16    & Grid              & action  & 1.36   \\
% VGG-16    & Grid              & object  & 2.67   \\
% ResNet-101 & Distribution     & action  & 2.26 \\
% ResNet-101 & Distribution     & object  & 3.43 \\
% ResNet-101 & Distribution ($\mu$)     & action+object  & 5.46 \\ 
% ResNet-101 & Distribution ($\sigma$)     & action+object  & 5.46 \\
% ResNet-101 & Distribution ($\mu + \sigma$)    & action+object  & \textbf{7.11} \\\hline
\end{tabular}
\vspace{-0.8\baselineskip}
\end{table}

The quantitative results of VGG-16 as the backbone network are presented in \tabref{tbl:ab_study} for different ablation settings. First, we observe that a learnable grid-based or normal distribution for the anchor location outperforms a simple heuristic choice of the image center as the anchor. We also see that the normal distribution, where both mean and variance are learned for each action-object pair leads to better results compared to the other settings. This validates our hypothesis that good modeling of the object spatial prior \wrt~human in an action provides strong cues for detection.

%proves the Comparing different correlation mechanisms, a large performance boost is achieved from pre-defined correlation (``center'') to a learnable model (``Grid''), proving the correlation is helpful for localizing the object and such correlation is learnable. Better performance is achieved by replacing the grid with a more fine designed learnable distribution. Another observation is from the comparison between learning $\mu$, $\sigma$ and $\mu+\sigma$ that learning all hyper-parameters in the distribution generates better performance, showing that the modeling spatial correlation is optimized by learning all the parameters.

We also notice that both the object classification and action classification modules contribute significantly to the final performance. Jointly modelling both action and object classification achieves the best result, validating our hypothesis that action classification and object detection can help each other.

We also visualize the learned distribution of object location probabilities from the prior module for a few sample videos/images in Fig. \ref{fig:distribution}. The learned distribution often has large probability weights around the object mentioned in the action. For example, in the first two columns of the visualization, it is much easier to localize the object with the cues from the heatmap. However, we also note that this distribution is less useful for actions where there is no consistent physical interaction between the human and the object. This is shown in the last column of the figure, for actions like ``watching television" and ``flying kite". Our approach reports relatively low mAP performance on such object classes (Tab. \ref{tbl:class_wise_charades} and Tab. \ref{tbl:class_wise_hico}).

\begin{figure}
\centering
\vspace{-0.4\baselineskip}
\includegraphics[width=0.45\textwidth]{figures/distribution.pdf}
\caption{Visualization of learned object location probability w.r.t. selected person keypoint. The heatmap represents the probability of object location (brighter color represents larger probability value) and the white circle represents the selected keypoint.}
\label{fig:distribution}
\vspace{-0.3\baselineskip}
\end{figure} 

\begin{figure}
% \vspace{-0.4\baselineskip}
\centering
\includegraphics[width=0.5\textwidth]{figures/ratio_exp2.pdf}
\caption{Performance comparison between our method trained in a semi-supervised setting, fully supervised setting and R*CNN trained in a semi-supervised approach on (a) Charades dataset and (b) HICO-DET dataset.}
\label{fig:semi-supervision}
\vspace{-1.0\baselineskip}
\end{figure}

\vspace{-0.5\baselineskip}
\subsection{Effect of supervision in training}
\vspace{-0.4\baselineskip}
\label{sec:supervision}

\begin{table*}[t]
\centering
\fontsize{8}{8.5}\selectfont
\caption{AP performance (\%) on each object class and mAP (\%) comparison with different weakly supervised methods on Charades.}
\label{tbl:class_wise_charades}
\def\arraystretch{1.1}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|ccccccccccccccccc|c}
\specialrule{.2em}{.1em}{.1em}
Methods                                        & bed & broom & chair & cup & dish & door & laptop & mirror & pillow & refri & shelf & sofa    & table   & tv   & towel       & vacuum    & window     & mAP(\%)      \\ \hline
WSDDN \cite{bilen2016weakly}                   & 2.38 & 0.04 &1.17 &0.03 & 0.13 & 0.31 & 2.81 & 0.28 & 0.02 & 0.12 & 0.03 & 0.41 & 1.74 & 1.18 & 0.07 & 0.08 & 0.22 & 0.65   \\
R*CNN \cite{gkioxari2015contextual}           & 2.17 & 0.44 & 2.03 & 0.31 & 0.08 & 0.77 & 2.64 & 0.32 & 1.24 & 2.36 & 0.82 & 1.41 & 0.65 & 0.72 & 0.07 & 0.65 & 0.17 & 0.99 \\
ContextLocNet \cite{kantorov2016contextlocnet} & 7.40 & 0.03 & 0.55 & 0.02 & 0.01 & 0.17 & 1.11 &0.66 & 0.00 & 0.07 & 1.75 & 4.12 & 0.63 & 0.99 & 0.03 & 0.75 & 0.78 & 1.12  \\
TD-LSTM \cite{yuan2017temporal}                & 9.19 & 0.04 & 4.18 & 0.49 & 0.11 & 1.17 & 2.91 & 0.30 & 0.08 & 0.29 & 3.21 & 5.86 & 3.35 & 1.27 & 0.09 & 0.60 & 0.47 & 1.98 \\ 
PCL \cite{tang2018pcl}                         & 4.62 & 1.07 & 2.21 & 1.26 & 1.08 & 2.49 & 3.61 & \textbf{5.13} & 1.34 & 4.46 & 3.29 & 5.61 & 3.84 & 3.26 & 1.17 & 1.43 & 2.27 & 2.83 \\
% PCL \cite{tang2018pcl}                         & 8.64 & 2.49 & 4.21 & 1.57 & 2.67 & 6.16 & 5.27 & 5.13 & 2.34 & 8.49 & 4.29 & 9.61 & 4.84 & 5.47 & 2.17 & 2.43 & 3.27 & 4.65 \\
R*CNN + prior                            & 6.82 & 3.64 & 5.39 & 3.25 & 2.47 & 3.36 & 5.27 & 1.07 & 2.38 & 6.34 & 3.29 & 5.72 & 4.09 & 1.03 & 1.26 & 3.41 & 0.86 & 3.50 \\
PCL + prior                                    & 10.57 & 5.63 & 8.24 & 3.52 & 3.71 & 5.63 & 6.86 & 4.96 & 5.23 & 11.39 & 4.88 & 10.46 & 6.32 & \textbf{3.53} & 4.06 & 4.89 & \textbf{3.07} & 6.05 \\
% PCL + prior                              & 11.27 & 5.93 & 9.24 & 4.02 & 4.31 & 6.53 & 6.06 & \textbf{4.96} & 5.23 & 12.39 & 5.88 & 12.46 & 7.82 & \textbf{5.53} & 4.06 & 5.89 & \textbf{4.07} & 6.76 \\
\hline
Ours (w/o prior)                         & 6.71 & 2.32 & 5.48 & 2.49 & 1.04 & 3.60 & 4.02 & 3.42 & 4.39 & 7.76 & 3.15 & 7.43 & 3.26 & 1.62 & 0.89 & 2.24 & 1.23 & 3.60\\ 
Ours (vgg-16)                                  & 14.92 & 10.23 & 13.08 & 7.65 & 5.21 & 6.44 & 8.65 & 4.79 & 9.14 & 18.07 & 7.29 & 17.21 & 8.46 & 2.37 & 5.46 & 7.23 & 2.64 & 8.76\\ 
Ours (ResNet-101)                              & \textbf{16.54} & \textbf{11.63} & \textbf{14.87} & \textbf{8.62} & \textbf{6.73} & \textbf{8.29} & \textbf{11.32} & \textbf{4.96} & \textbf{9.81} & \textbf{19.24} & \textbf{9.03} & \textbf{18.49} & \textbf{9.86} & 3.05 & \textbf{6.48} & \textbf{8.08} & 3.02 & \textbf{10.03}\\\hline
\end{tabular}
\vspace{-0.4\baselineskip}
\end{table*}

\begin{figure*}
\vspace{-0.2\baselineskip}
\centering
\includegraphics[width=0.95\textwidth]{figures/det2.pdf}
\caption{Qualitative detection results on (a) Charades test frames and (b) HICO-DET test images. Red bounding boxes denote our results and green bounding boxes denote results of PCL \cite{tang2018pcl}}
\label{fig:det_vis}
\vspace{-1.2\baselineskip}
\end{figure*} 

In order to fully understand the utility of our method, we also explore the results of our model in a more practical setting, where bounding box annotations maybe available for a small number of videos or images during training. This is similar to a semi-supervised setting. We explore the effect of adding varying amounts of ground truth object bounding box annotations into our training data. Besides the losses described in Sec. \ref{sec:approach}, an additional supervised object classification loss is added for training videos/images where these annotations are available. In practice, the IoU between object proposals and ground truth object bounding boxes is calculated and proposals having higher IoU than the threshold are considered positive samples and rest as negative. The threshold IoU is set as 0.45 to guarantee a reasonable positive samples per image. The negative and positive sample ratio is set as 5. 

We compare with two baseline methods: (1) a fully supervised variant of our approach: our approach trained with only supervised object classification loss and (2)R*CNN \cite{gkioxari2015contextual} with additional object bounding box supervision as above. We chose to compare with the R*CNN variant as it leverages similar supervision signals and can be easily adapted to a semi-supervised setting.


The semi-supervised setup is evaluated on both Charades and HICO-DET datasets. The quantitative results are presented in Fig. \ref{fig:semi-supervision}. The x-axis (log scale) represents the percentage of available training samples for whom we assume full supervision. For example, the point $x\%$ represents that for a random $x\%$ of training data samples we assume the bounding box annotations are present. For the remaining training samples, only action class label information is used. Note that $0\%$ is the weakly-supervised setting considered earlier, while $100\%$ represents fully-supervised setting. We observe that the mAP increases log-linearly as the supervision is added to the training.

%Notice that at ``0\%'', weakly supervised method (ours and R*CNN) outperforms the fully supervised baseline as these two methods can still learn the object representation without explicit object labels. 

For Charades, when small amount of supervision is used, we observe that our weakly-supervised approach significantly outperforms the fully-supervised setting. This clearly shows the potential of our weakly-supervised approach to provide complementary value in the low shot detection setting. With as low as 70\% supervision, our semi-supervised approach already matches the performance of fully-supervised method at 100\% supervision. As expected, the gap between the two approaches decrease with increase in supervision. This is because bounding box labels provide strong supervision and thus the performance boost from action labels (weak supervision) is overwhelmed. Nevertheless, even with ``100\%'' bounding box annotations, the semi-supervised method still outperforms the fully supervised method by $2-3$ mAP points. In contrast, R*CNN variant achieves very marginal gains over fully-supervised setting that quickly vanish with increase in supervision.
We also observe that performance gap is noticeably smaller for HICO-DET. This is because the advantage of weak supervision is stronger in the case of videos, where temporal linking of proposals helps in avoiding spurious detections during training.

\begin{table*}[]
\vspace{-0.5\baselineskip}
\centering
\fontsize{8.5}{9}\selectfont
\caption{AP performance (\%) on selected object classes and mAP (\%) comparison with other weakly supervised methods on HICO-DET.}
\label{tbl:class_wise_hico}
\def\arraystretch{1.1}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccccccccc|c}
\specialrule{.2em}{.1em}{.1em}
Methods & apple & bicycle & bottle & chair & cellphone & frisbee & kite & surfboard & train & umbrella & mAP(\%)      \\ \hline
R*CNN \cite{gkioxari2015contextual}   & 1.13 & 3.26 & 1.57 & 2.35 & 1.47 & 1.02& 0.32 & 2.70 & 2.86 & 3.04 & 2.15 \\ 
WSDDN \cite{bilen2016weakly}  & 1.46 & 5.19 & 1.52 & 3.87 & 2.02 & 2.44 & 1.15 & 2.86 & 6.76 & 3.35 & 3.27   \\
PCL \cite{tang2018pcl}          & 1.27 & 5.82 & 2.31 & 2.84 & 3.06 & \textbf{3.11}& 1.16 & 2.60 & 7.93 & 3.47 & 3.62 \\ 
PCL + prior                 & 2.06 & 6.49 & 2.54 & 3.69 & 5.14 & 2.96 & \textbf{1.37} & 4.06 & 8.13 & 4.87 & 4.19 \\
\hline
Ours (w/o prior)                    & 1.23 & 5.15 & 1.19 & 3.47 & 3.82 & 2.24 & 0.73 & 3.65 & 6.22 & 3.14 & 3.16\\
Ours (vgg-16)                       & \textbf{2.47} & \textbf{8.64} & \textbf{3.59} & \textbf{5.74} & \textbf{7.36} & 2.85 & 0.87 & \textbf{7.29} & \textbf{8.47} & \textbf{6.63} & \textbf{5.39}\\ \hline
\end{tabular}
\vspace{-1.2\baselineskip}
\end{table*}

\vspace{-0.6\baselineskip}
\subsection{Comparison with existing methods}
\vspace{-0.4\baselineskip}
In this section, we compare our method with other weakly supervised methods and their variants: (1) WSDDN \cite{bilen2016weakly}; (2) ContextLocNet \cite{kantorov2016contextlocnet}; (3) PCL \cite{tang2018pcl}; action-driven weakly supervised object detection method: (4) TD-LSTM \cite{yuan2017temporal} and (5) R*CNN \cite{gkioxari2015contextual} which is designed for action recognition with awareness of the main object. We used the main object bounding box as the object detection result. R*CNN is pre-trained on Pascal-action dataset and then finetuned on Charades or HICO-DET dataset. Note that the (1), (2), (3), (4) do not use person bounding box or keypoint detection results in their model unlike our method. While (5) uses person bounding box, it doesn't use person keypoints. In order to enable fair comparison with other methods, we also construct another variant of PCL and R*CNN which uses keypoints: (6) R*CNN with spatial prior and (7) PCL with spatial prior, where we replace the max pooling in R*CNN and mean pooling in PCL with a weighted sum where the weights are computed from spatial prior distribution as in our implementation (more details are presented in supplemental material). 

Results from TD-LSTM \cite{yuan2017temporal} are shown only for Charades, since it is a video-specific model and code is not available. Also, we report results from weakly-supervised models whose code is available or whose results on Charades, HICO-DET or EPIC KITCHENS datasets is readily available. Also, note that many methods such as \cite{diba2017weakly,wei2018ts2c,bai2017multiple} are built on top of the vanilla WSDDN method by adding signals such as segmentation, contextual information, instance refinement, \etc and these ideas are complementary to the ones presented in this work, and can be added to our model to achiever better results.
The per-class AP and combined mAP performances on the two datasets are presented in Tab. \ref{tbl:class_wise_charades} and Tab. \ref{tbl:class_wise_hico} respectively. 10 object classes on HICO-DET are randomly selected and presented.

On Charades dataset, our method achieves 6\% mAP boost compared to PCL \cite{tang2018pcl}. Our method performs significantly better on object classes like broom, refrigerator, vacuum, \etc. The spatial prior patterns of the interactions involving these object classes are more predictable and thus the prior modeling benefits our approach more than on other object classes. For object like tv, the spatial prior pattern of the interaction (\eg \textit{watch tv}) is more diverse and thus difficult to model, resulting only a small boost in mAP. The same performance pattern also applies to HICO-DET dataset. On the object class kite, our method slightly performs inferior to the baseline method.

\begin{table}[]
\vspace{-0.2\baselineskip}
\centering
\fontsize{8.5}{9}\selectfont
\caption{Weakly supervised object detection performances on EPIC KITCHENS}
\label{tbl:epic}
\def\arraystretch{1.2}
\begin{tabular}{l|cc}
\specialrule{.2em}{.1em}{.1em}
Methods                        & mAP  & CorLoc\\ \cline{1-3}
R*CNN \cite{gkioxari2015contextual} & 2.54 & 32.68  \\
PCL \cite{tang2018pcl}   & 4.68 & 40.64 \\
PCL + prior  & 6.82 & 46.69  \\ \cline{1-3}
Ours                           & \textbf{9.75} & \textbf{52.53}  \\ \cline{1-3}
\end{tabular}
\vspace{-1.8\baselineskip}
\end{table}

We observe that the spatial prior from our model is effective in localizing the object during training even when combined with other models such as R*CNN \cite{gkioxari2015contextual} and PCL \cite{tang2018pcl}. R*CNN with spatial prior modeling outperforms TD-LSTM, which is specifically designed for the action driven weakly supervised object detection task.
% , and also outperforms the original R*CNN by a large margin, validating the effectiveness of the object spatial prior. 
We also report our method without spatial prior module (ours (w/o prior)). As object and action informations are jointly modeled in our approach, our degenerated approach still outperforms TD-LSTM on Charades.
The qualitative comparison between our method and PCL is presented in Fig. \ref{fig:det_vis}. Our approach localizes the object more accurately. Multiple object classes and multiple instances can be detected through our trained object classification stream. The last column shows our failure cases. On Charades, both PCL \cite{tang2018pcl} and our method fail to detect the windows and on HICO-DET, our method fails to localize the kite. One possible reason is that Window has very diverse appearance and also the interaction pattern between human and object (watch out of the window, \etc) is difficult to model.

Our approach can be easily extended to ego-centric data. The EPIC KITCHENS dataset is capturing daily kitchen activities with head-mounted camera and the human is not visible in the video. We applied the framework with ``center'' spatial prior modeling: assume the frame center to be the anchor location and estimate distribution parameters \wrt~ the central location. As the camera is fixed with respect to the human body, we believe the anchor location is already implicitly modeled within the video. We compare with R*CNN \cite{gkioxari2015contextual} and PCL \cite{tang2018pcl} on the 1,200 test frames using mAP metric. 

Although the human keypoints are not visible and thus cannot be detected on this dataset, the first-person vision provides a strong prior for the spatial locations and thus our method is able to outperform the two weakly supervised weakly supervised methods as in Tab. \ref{tbl:epic}. More detailed results (per-class AP) are reported in the supplemental material.
